NTIRE 2025 Image Shadow Removal Challenge Report

This work examines the findings of the NTIRE 2025 Shadow Removal Challenge. A total of 306 participants have registered, with 17 teams successfully submitting their solutions during the final evaluation phase. Following the last two editions, this challenge had two evaluation tracks: one focusing on reconstruction fidelity and the other on visual perception through a user study. Both tracks were evaluated with images from the WSRD+ dataset, simulating interactions between self- and cast-shadows with a large number of diverse objects, textures, and materials.

==> teams/Oath/include.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{teams/Oath/tex/dualreti_shadow_f_re-compressed.pdf}
    \caption{Overfiew of the dual branch architecture proposed by Oath. One branch restores reflectance while the other restores illumination information.
    %The overall architecture of our model. There are two branches in our method, and each is designed to restore the reflectance and illumination information. Besides, we develop a CNN-Transformer Hybrid Module as the primary restoration network. Specifically, the retinex-guided Histogram Transformer block is propose to dynamically perceive the and process the shadow region.
    }
    \label{fig:Oath}
    \vspace{-3mm}
\end{figure}

\subsection{Oath}
% A lightweight Retinex-guided CNN-Transformer Hybrid model for Shadow Removal task.
The solution proposed by Oath employs Retinex theory~\cite{land1977retinex} and a dual-branch Illumination-Guided Shadow Removal framework.
Retinex theory plays a crucial role in shadow removal by providing a framework for separating reflectance (intrinsic object colors) from illumination variations. 
In the proposed architecture shown in \fref{fig:Oath} after separating reflectance and illuminance through the Retinex estimator, each is individually processed by one branch of the network.
Each branch is a Illumination-Guided Hybrid CNN-Transformers (IG-HCT) module composed of multiple IG-HCT blocks (IG-HCTB) each containing a Dilated Residual Dense Block (DRDB), an Illumination-Guided Histogram Transformer Block (IG-HTB), and a Semantic-aligned scale-aware module (SAM) to boost the network’s capability in handling shadow patterns with diverse scales without incurring too much computational cost. 
The illumination-guided design of IG-HTB is inspired by RetinexFormer~\cite{cai2023retinexformer}. 
This block is composed of two-layer normalization (LN), an Illumination-Guided Histogram Self-Attention (IG-HSA) module, and a feed-forward network (FFN).

